Material Decomposition in Photon-Counting Computed Tomography with Diffusion Models: Comparative Study and Hybridization with Variational Regularizers

Photon-counting computed tomography (PCCT) has emerged as a promising imaging technique, enabling spectral imaging and material decomposition (MD). However, images typically suffer from a low signal-to-noise ratio (SNR) due to constraints such as low photon counts and sparse-view settings which provoke artifacts. To prevent this, variational methods minimize a data-fit function coupled with handcrafted regularizers that mimic a prior by enforcing image properties such as gradient sparsity. In the last few years, diffusion models (DMs) have become predominant in the field of generative models and have been used as a learned prior for image reconstruction. This work investigates the use of DMs as regularizers for MD tasks in PCCT, specifically using diffusion posterior sampling (DPS) guidance. Three DPS-based approaches -- image-domain two-step DPS (im-TDPS), projection-domain two-step DPS (proj-TDPS), and one-step DPS (ODPS) -- are evaluated. The first two methods achieve MD in two steps by performing reconstruction and MD separately. The last method, ODPS, samples the material images directly from the measurement data. The results indicate that ODPS achieves superior performance compared to im-TDPS and proj-TDPS, providing sharper, noise-free and crosstalk-free images. Furthermore, we introduce a novel hybrid method for scenarios involving materials absent from the training dataset which combines DM priors with standard variational handcrafted regularizers for the materials unknown to the DM. This hybrid method demonstrates improved MD quality compared to a standard variational method and does not require additional training of the DM neural network (NN).

==> figures/macros.tex <==
\newcommand{\bolda}{\bm{a}}
\newcommand{\boldb}{\bm{b}}
\newcommand{\boldc}{\bm{c}}
\newcommand{\boldd}{\bm{d}}
\newcommand{\bolde}{\bm{e}}
\newcommand{\boldf}{\bm{f}}
\newcommand{\boldg}{\bm{g}}
\newcommand{\boldh}{\bm{h}}
\newcommand{\boldi}{\bm{i}}
\newcommand{\boldj}{\bm{j}}
\newcommand{\boldk}{\bm{k}}
\newcommand{\boldl}{\bm{l}}
\newcommand{\boldm}{\bm{m}}
\newcommand{\boldn}{\bm{n}}
\newcommand{\boldo}{\bm{o}}
\newcommand{\boldp}{\bm{p}}
\newcommand{\boldq}{\bm{q}}
\newcommand{\boldr}{\bm{r}}
\newcommand{\bolds}{\bm{s}}
\newcommand{\boldt}{\bm{t}}
\newcommand{\boldu}{\bm{u}}
\newcommand{\boldv}{\bm{v}}
\newcommand{\boldw}{\bm{w}}
\newcommand{\boldx}{\bm{x}}
\newcommand{\boldy}{\bm{y}}
\newcommand{\boldz}{\bm{z}}

\newcommand{\boldlambda}{\bm{\lambda}}
\newcommand{\boldmu}{\bm{\mu}}




\newcommand{\boldA}{\bm{A}}
\newcommand{\boldB}{\bm{B}}
\newcommand{\boldC}{\bm{C}}
\newcommand{\boldD}{\bm{D}}
\newcommand{\boldE}{\bm{E}}
\newcommand{\boldF}{\bm{F}}
\newcommand{\boldG}{\bm{G}}
\newcommand{\boldH}{\bm{H}}
\newcommand{\boldI}{\bm{I}}
\newcommand{\boldJ}{\bm{J}}
\newcommand{\boldK}{\bm{K}}
\newcommand{\boldL}{\bm{L}}
\newcommand{\boldM}{\bm{M}}
\newcommand{\boldN}{\bm{N}}
\newcommand{\boldO}{\bm{O}}
\newcommand{\boldP}{\bm{P}}
\newcommand{\boldQ}{\bm{Q}}
\newcommand{\boldR}{\bm{R}}
\newcommand{\boldS}{\bm{S}}
\newcommand{\boldT}{\bm{T}}
\newcommand{\boldU}{\bm{U}}
\newcommand{\boldV}{\bm{V}}
\newcommand{\boldW}{\bm{W}}
\newcommand{\boldX}{\bm{X}}
\newcommand{\boldY}{\bm{Y}}
\newcommand{\boldZ}{\bm{Z}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}


\newcommand{\boldcalA}{\bm{\mathcal{A}}}
\newcommand{\boldcalB}{\bm{\mathcal{B}}}
\newcommand{\boldcalC}{\bm{\mathcal{C}}}
\newcommand{\boldcalD}{\bm{\mathcal{D}}}
\newcommand{\boldcalE}{\bm{\mathcal{E}}}
\newcommand{\boldcalF}{\bm{\mathcal{F}}}
\newcommand{\boldcalG}{\bm{\mathcal{G}}}
\newcommand{\boldcalH}{\bm{\mathcal{H}}}
\newcommand{\boldcalI}{\bm{\mathcal{I}}}
\newcommand{\boldcalJ}{\bm{\mathcal{J}}}
\newcommand{\boldcalK}{\bm{\mathcal{K}}}
\newcommand{\boldcalL}{\bm{\mathcal{L}}}
\newcommand{\boldcalM}{\bm{\mathcal{M}}}
\newcommand{\boldcalN}{\bm{\mathcal{N}}}
\newcommand{\boldcalO}{\bm{\mathcal{O}}}
\newcommand{\boldcalP}{\bm{\mathcal{P}}}
\newcommand{\boldcalQ}{\bm{\mathcal{Q}}}
\newcommand{\boldcalR}{\bm{\mathcal{R}}}
\newcommand{\boldcalS}{\bm{\mathcal{S}}}
\newcommand{\boldcalT}{\bm{\mathcal{T}}}
\newcommand{\boldcalU}{\bm{\mathcal{U}}}
\newcommand{\boldcalV}{\bm{\mathcal{V}}}
\newcommand{\boldcalW}{\bm{\mathcal{W}}}
\newcommand{\boldcalX}{\bm{\mathcal{X}}}
\newcommand{\boldcalY}{\bm{\mathcal{Y}}}
\newcommand{\boldcalZ}{\bm{\mathcal{Z}}}



\newcommand{\rma}{\mathrm{a}}
\newcommand{\rmb}{\mathrm{b}}
\newcommand{\rmc}{\mathrm{c}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmf}{\mathrm{f}}
\newcommand{\rmg}{\mathrm{g}}
\newcommand{\rmh}{\mathrm{h}}
\newcommand{\rmi}{\mathrm{i}}
\newcommand{\rmj}{\mathrm{j}}
\newcommand{\rmk}{\mathrm{k}}
\newcommand{\rml}{\mathrm{l}}
\newcommand{\rmm}{\mathrm{m}}
\newcommand{\rmn}{\mathrm{n}}
\newcommand{\rmo}{\mathrm{o}}
\newcommand{\rmp}{\mathrm{p}}
\newcommand{\rmq}{\mathrm{q}}
\newcommand{\rmr}{\mathrm{r}}
\newcommand{\rms}{\mathrm{s}}
\newcommand{\rmt}{\mathrm{t}}
\newcommand{\rmu}{\mathrm{u}}
\newcommand{\rmv}{\mathrm{v}}
\newcommand{\rmw}{\mathrm{w}}
\newcommand{\rmx}{\mathrm{x}}
\newcommand{\rmy}{\mathrm{y}}
\newcommand{\rmz}{\mathrm{z}}

\newcommand{\rmA}{\mathrm{A}}
\newcommand{\rmB}{\mathrm{B}}
\newcommand{\rmC}{\mathrm{C}}
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\rmE}{\mathrm{E}}
\newcommand{\rmF}{\mathrm{F}}
\newcommand{\rmG}{\mathrm{G}}
\newcommand{\rmH}{\mathrm{H}}
\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmJ}{\mathrm{J}}
\newcommand{\rmK}{\mathrm{K}}
\newcommand{\rmL}{\mathrm{L}}
\newcommand{\rmM}{\mathrm{M}}
\newcommand{\rmN}{\mathrm{N}}
\newcommand{\rmO}{\mathrm{O}}
\newcommand{\rmP}{\mathrm{P}}
\newcommand{\rmQ}{\mathrm{Q}}
\newcommand{\rmR}{\mathrm{R}}
\newcommand{\rmS}{\mathrm{S}}
\newcommand{\rmT}{\mathrm{T}}
\newcommand{\rmU}{\mathrm{U}}
\newcommand{\rmV}{\mathrm{V}}
\newcommand{\rmW}{\mathrm{W}}
\newcommand{\rmX}{\mathrm{X}}
\newcommand{\rmY}{\mathrm{Y}}
\newcommand{\rmZ}{\mathrm{Z}}


\newcommand{\R}{\mathbb{R}}
\newcommand{\transp}{^\top}

\newcommand{\xbar}{\bar{x}}
\newcommand{\boldxbar}{\bar{\boldx}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\boldybar}{\bar{\boldy}}
\newcommand{\zbar}{\bar{z}}
\newcommand{\boldzbar}{\bar{\boldz}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\boldgbar}{\bar{\boldg}}
\newcommand{\boldxhat}{\hat{\boldx}}
\newcommand{\boldxcheck}{\check{\boldx}}
\newcommand{\boldzhat}{\hat{\boldz}}

\newcommand{\boldtheta}{\bm{\theta}}
\newcommand{\boldsigma}{\bm{\sigma}}
\newcommand{\boldSigma}{\bm{\Sigma}}
\newcommand{\boldpsi}{\bm{\psi}}
\newcommand{\boldphi}{\bm{\phi}}
\newcommand{\boldTheta}{\bm{\Theta}}


\newcommand{\boldmuhat}{\hat{\boldmu}}
\newcommand{\boldmutilde}{\tilde{\boldmu}}
\newcommand{\boldlambdahat}{\hat{\boldlambda}}
\newcommand{\boldlambdatilde}{\tilde{\boldlambda}}
\newcommand{\boldeps}{\bm{\epsilon}}

\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}

\newcommand{\boldzero}{\bm{0}}

\algnewcommand{\Inputs}[1]{%
	\State \textbf{Inputs:}
	\Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Initialize}[1]{%
	\State \textbf{Initialize:}
	\Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}



==> figures/preamble.tex <==
% basics
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{breqn}
%\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{array}
%\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\usepackage{textcomp}
\usepackage{stfloats}
\usepackage{url}
\usepackage{verbatim}
\usepackage{graphicx}
%\usepackage{subfig}
\usepackage{stmaryrd}
\usepackage{microtype}
\usepackage{datatool}
\usepackage{siunitx}
\usepackage{pgf}

%\usepackage{tabularray}


\usepackage{bm} % bold math
\usepackage{lipsum}



\usepackage{acro} % acronyms
%\acsetup{list/template=tabularray}
\acsetup{single}
\usepackage{bm}
\usepackage{amsfonts}
\usepackage{soul}

% 
\usepackage[
	style=ieee,
	dashed=false,
	maxbibnames=20,
	minbibnames=2,
	maxcitenames=1,
	mincitenames=1,
	backend=biber,
	%defernumbers=true,
	sorting=none,
	useprefix=false
	]{biblatex}



\usepackage{tikz}
\usepackage{overpic}

\usetikzlibrary{arrows.meta,shapes,intersections,calc,angles,decorations.pathreplacing,intersections,quotes,angles,positioning,fit,petri,through,shadows,plotmarks,spy}


\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usetikzlibrary{pgfplots.groupplots}

\usepackage{algpseudocode}

\usepackage{caption}
\usepackage{subcaption}
\usepackage[labelformat=simple,font=footnotesize]{subcaption}
%\renewcommand\thesubfigure{(\alph{subfigure})}
\usepackage[font=small]{caption}
\captionsetup{subrefformat=parens}

\pdfoutput=1
